The Mega-MUSCLES Treasury Survey: X-ray to infrared Spectral Energy Distributions of a representative sample of M dwarfs

We present 5-1x10^7 Angstrom spectral energy distributions (SEDs) for twelve M dwarf stars covering spectral types M0-M8. Our SEDs are provided for community use as a sequel to the Measurements of the Ultraviolet Spectral Characteristics of Low-mass Exoplanetary Systems (MUSCLES) survey. The twelve stars include eight known exoplanet hosts and four stars chosen to fill out key parameter space in spectral type and rotation period. The SEDs are constructed from Hubble Space Telescope ultraviolet spectroscopy and XMM Newton, Chandra and/or Swift X-ray observations and completed with various model data, including Lyman alpha reconstructions, PHOENIX optical models, APEC coronal models and Differential Emission Measure models in the currently-unobservable Extreme Ultraviolet. We provide a complete overview of the Mega-MUSCLES program, including a description of the observations, models, and SED construction. The SEDs are available as MAST High-Level Science Products and we describe the various data products here. We also present ensemble measurements from our sample that are of particular relevance to exoplanet science, including the high-energy fluxes in the habitable zone and the FUV/NUV ratio. Combined with MUSCLES, Mega-MUSCLES provides SEDs covering a wide range of M\,dwarf spectral types and ages such that suitable proxies for any M dwarf planet host of interest may be found in our sample. However, we find that ultraviolet and X-ray fluxes can vary even between stars with similar parameters, such that observations of each exoplanet host star will remain the gold standard for interpreting exoplanet atmosphere observations.

==> archive_table.tex <==
\begin{table}
    \centering
    \begin{tabular}{lcc}
    \hline
    \hline
Name & CASLEO & X-shooter \\ \hline
TRAPPIST-1 & N & N \\
L-980-5 & N & N \\
GJ674 & Y & N \\
GJ676A & N & Y \\
GJ649 & N & N \\
GJ699 & Y & N \\
GJ163 & N & Y \\
GJ849 & N & Y \\
GJ1132 & N & N \\
LHS-2686 & N & N \\
GJ729 & Y & Y \\
GJ15A & N & N \\ \hline
    \end{tabular}
    \caption{\label{tab:archopt} Ground based optical spectra used to asses the flux calibration of the G430L spectra.}
    
\end{table}

==> big_targets_table.tex <==
\begin{deluxetable}{lcccccccccccc}
\tablecaption{Mega-MUSCLES Target Summary \label{tab_targs}}

\tabletypesize{\small}
\tablecolumns{8}
\tablehead{\colhead{Star} & \colhead{Distance} & \colhead{Spectral} & \colhead{M$_{\star}$} & \colhead{P$_{Rot}$} & \colhead{Exoplanet Mass} & \colhead{Semi-major Axis} & \colhead{Active?\tablenotemark{a}} & \colhead{Refs} \\
& \colhead{(pc)} & \colhead{Type} & \colhead{(\Msun)} & \colhead{days} & \colhead{(\mearth)} & \colhead{(AU)} }
\startdata
GJ676A & 16.0 & M0 V & 0.631 & 41.2 & 4.4\tablenotemark{b}, 11.5\tablenotemark{b}, 2127, 2161\tablenotemark{b} & 0.04, 0.187, 1.8152,6.6 &  N & 1 \\
GJ15A & 3.6 & M2 V & 0.393 & 30.5 & 5.35\tablenotemark{b} & 0.072 & N & 2,3, 18 \\
GJ649 & 10.4 & M1 V & 0.524 & 23.8 & 87.4\tablenotemark{b} & 1.13 & N & 4,5,19,20 \\
GJ674 & 4.6 & M3 V & 0.353 & 32.9 & 11.1\tablenotemark{b} & 0.039 & N & 6,7,21 \\
GJ729 & 3.0 & M3.5 V & 0.177 & 2.8 & & & Y & 2,3,8 \\
GJ163 & 15.1 & M3.5 V & 0.405 & 61 & 10.6\tablenotemark{b}, 6.8\tablenotemark{b}, 29.0\tablenotemark{b} & 0.061, 0.125, 1.03 & N & 1,9 \\
GJ1132 & 12.6 & M4 V & 0.194 & 126.6 & 1.66,2.64\tablenotemark{b} & 0.0153,0.0476 & N & 10,11,22 \\
L980-5 & 13.3 & M4 V & 0.232 & 92.2 & & & N & 11\\
GJ849 & 8.8 & M3.5 V & 0.524 & 39.2 & 283\tablenotemark{b}, 342.9\tablenotemark{b} & 2.409, 4.974 & N & 1,5,20,23,24  \\
GJ699 & 1.8 & M4 V & 0.161 & 130.4 & 0.37\tablenotemark{b} & 0.02294 & N & 12,13 \\
%LP756-18 & 12.1 & M5 & 128.2 & & & N \\
LHS2686 & 12.2 & M5 V & 0.157 & 28.8 & & & Y \\
Trappist-1 & 12.1 & M7.5 V & 0.090 & 3.3 & 1.017, 1.156, 0.297 & 0.011, 0.015, 0.022 & Y & 14,15,25,26 \\
& & & & &  0.772, 0.934 & 0.029, 0.039  \\
& & & & & 1.148, 0.331 & 0.047, 0.062  \\
\enddata
\tablecomments{Distances taken from Gaia DR2 \citep{gaia18-1,gaia16-1}. Stellar masses and spectral types taken from \citep{pinedaetal21-1}.  Rotational period references: 1 \citep{suarezmascarenoetal15-1}, 2 \citep{newtonetal16-1}, 3 \citep{allenandherrera98-1}, 4 \citep{diezalonsoetal19-1}, 5 \citep{veyette+muirhead18-1}, 6 \citep{kiraga+stepien07-1}, 7 \citep{montesetal01-1},  8 \citep{ibanezbustosetal20-1}, 9 \citep{bonfilsetal13-1}, 10 \citep{newtonetal18-1},11 \citep{bertathompsonetal15-1}, 12 \citep{toledopadronetal19-1}, 13 \citep{ribasetal18-1}, 14 \citep{vidaetal17-1}, 15 \citep{burgasser+mamajek17-1}. Exoplanet properties references: 16 \citep{angladaescude+tuomi12-1}, 17 \citep{sahlmannetal16-1}, 18 \citep{howardetal14-1}, 19 \citep{johnsonetal10-1}, 20 \citep{rosenthatetal21-1}, 21 \citep{bonfilsetal07-1}, 22 \citep{bonfilsetal18-1}, 23 \citep{butleretal06-1}, 24 \citep{montetetal14-1}, 25 \citep{gillonetal16-1}. 26 \citep{grimetal18-1} }
\tablenotetext{a}{Optical activity designation where ``Y'' (Yes) indicates targets for which H$\alpha$ is in emission \citep{newtonetal17-1} }
\tablenotetext{b}{M$\sin i$ }
\end{deluxetable}

\begin{table}[]
    \centering
    \begin{tabular}{l c c c c } \hline \hline
     Name & $L_{\mathrm{bol}}$ (10$^{31}$ erg s$^{-1}$)  & Mass ($M_{\odot}$) & Radius ($R_{\odot}$) & $T_{\mathrm{eff}}$ (K) \\ \hline
	TRAPPIST-1 & $0.234 \pm ^{0.009}_{0.008}$ & $0.090 \pm ^{0.003}_{0.002}$ & $0.120 \pm 0.006 $ & $2619 \pm ^{71}_{66}$ \\ 
	LHS 2686 & $1.078 \pm 0.024$ & $0.157 \pm 0.004$ & $0.182 \pm 0.008 $ & $3119 \pm ^{70}_{68}$ \\ 
	GJ 699  & $1.302 \pm ^{0.024}_{0.023}$ & $0.1610 \pm ^{0.0036}_{0.0035} $ & $0.187 \pm 0.001$ & $3223 \pm 17 $ \\ 
	GJ 729 & $1.537 \pm 0.018$ & $0.177 \pm 0.004 $ & $0.200 \pm 0.008 $ & $3248 \pm ^{68}_{66}$ \\ 
	GJ 1132 & $1.668 \pm ^{0.049}_{0.047}$ & $0.194 \pm 0.005$ & $0.215 \pm 0.009$ & $3196 \pm ^{71}_{70}$ \\ 
	L 980-5 & $2.488 \pm ^{0.079}_{0.078}$ & $0.232 \pm 0.006$ & $0.250 \pm 0.010$ & $3278 \pm ^{74}_{70}$ \\ 
	GJ 674  & $6.03 \pm 0.14 $ & $0.353 \pm 0.008$ & $0.361 \pm ^{0.012}_{0.011}$ & $3404 \pm ^{59}_{57}$ \\ 
	GJ 15A  & $8.608 \pm 0.069$ & $0.393 \pm ^{0.009}_{0.008}$ & $0.385 \pm0.002$ & $3601 \pm ^{12}_{11}$ \\ 
	GJ 163 & $8.28 \pm 0.24$ & $0.405 \pm 0.010 $ & $0.409 \pm ^{0.017}_{0.016}$ & $3460 \pm ^{76}_{74}$ \\ 
	GJ 849 & $11.051 \pm ^{0.095}_{0.094}$ & $0.465 \pm 0.011$ & $0.464 \pm 0.018$ & $3492 \pm ^{70}_{68}$ \\ 
	GJ 649  & $16.74 \pm 0.170 $ & $0.524 \pm 0.012 $ & $0.531 \pm 0.012 $ & $3621 \pm ^{41}_{40}$ \\ 
	GJ 676A & $34.04 \pm ^{0.84}_{0.80}$ & $0.631 \pm 0.017$ & $0.617 \pm ^{0.028}_{0.027}$ & $4014 \pm ^{94}_{90}$ \\ \hline
    \end{tabular}
    \caption{Stellar parameters for the Mega-MUSCLES sample reproduced from Table 3 of \citet{pinedaetal21-1}.}
    \label{tab:params}
\end{table}





\begin{deluxetable}{lcccccccc}
\tablecaption{Mega-MUSCLES Target Summary \label{tab_targs}}

\tabletypesize{\small}
\tablecolumns{8}
\tablehead{\colhead{Star} & \colhead{Distance} & \colhead{Spectral} & \colhead{M$_{\star}$} & \colhead{P$_{Rot}$} & \colhead{Exoplanet Mass} & \colhead{Semi-major Axis} & \colhead{Active?\tablenotemark{a}} & \colhead{Refs} \\
& \colhead{(pc)} & \colhead{Type} & \colhead{(\Msun)} & \colhead{days} & \colhead{(\mearth)} & \colhead{(AU)} }
\startdata
GJ676A & 16.0 & M0 V & 0.631 & 41.2 & 4.4\tablenotemark{b}, 11.5\tablenotemark{b}, 2127, 2161\tablenotemark{b} & 0.04, 0.187, 1.8152,6.6 &  N & 1 \\
GJ15A & 3.6 & M2 V & 0.393 & 30.5 & 5.35\tablenotemark{b} & 0.072 & N & 2,3, 18 \\
GJ649 & 10.4 & M1 V & 0.524 & 23.8 & 87.4\tablenotemark{b} & 1.13 & N & 4,5,19,20 \\
GJ674 & 4.6 & M3 V & 0.353 & 32.9 & 11.1\tablenotemark{b} & 0.039 & N & 6,7,21 \\
GJ729 & 3.0 & M3.5 V & 0.177 & 2.8 & & & Y & 2,3,8 \\
GJ163 & 15.1 & M3.5 V & 0.405 & 61 & 10.6\tablenotemark{b}, 6.8\tablenotemark{b}, 29.0\tablenotemark{b} & 0.061, 0.125, 1.03 & N & 1,9 \\
GJ1132 & 12.6 & M4 V & 0.194 & 126.6 & 1.66,2.64\tablenotemark{b} & 0.0153,0.0476 & N & 10,11,22 \\
L980-5 & 13.3 & M4 V & 0.232 & 92.2 & & & N & 11\\
GJ849 & 8.8 & M3.5 V & 0.524 & 39.2 & 283\tablenotemark{b}, 342.9\tablenotemark{b} & 2.409, 4.974 & N & 1,5,20,23,24  \\
GJ699 & 1.8 & M4 V & 0.161 & 130.4 & & & N & 12,13 \\
%LP756-18 & 12.1 & M5 & 128.2 & & & N \\
LHS2686 & 12.2 & M5 V & 0.157 & 28.8 & & & Y \\
Trappist-1 & 12.1 & M7.5 V & 0.090 & 3.3 & 1.017, 1.156, 0.297 & 0.011, 0.015, 0.022 & Y & 14,15,25,26 \\
& & & & &  0.772, 0.934 & 0.029, 0.039  \\
& & & & & 1.148, 0.331 & 0.047, 0.062  \\
\enddata
\tablecomments{Distances taken from Gaia DR2 \citep{gaia18-1,gaia16-1}. Stellar masses and spectral types taken from \citep{pinedaetal21-1}.  Rotational period references: 1 \citep{suarezmascarenoetal15-1}, 2 \citep{newtonetal16-1}, 3 \citep{allenandherrera98-1}, 4 \citep{diezalonsoetal19-1}, 5 \citep{veyette+muirhead18-1}, 6 \citep{kiraga+stepien07-1}, 7 \citep{montesetal01-1},  8 \citep{ibanezbustosetal20-1}, 9 \citep{bonfilsetal13-1}, 10 \citep{newtonetal18-1},11 \citep{bertathompsonetal15-1}, 12 \citep{toledopadronetal19-1}, 13 \citep{ribasetal18-1}, 14 \citep{vidaetal17-1}, 15 \citep{burgasser+mamajek17-1}. Exoplanet properties references: 16 \citep{angladaescude+tuomi12-1}, 17 \citep{sahlmannetal16-1}, 18 \citep{howardetal14-1}, 19 \citep{johnsonetal10-1}, 20 \citep{rosenthatetal21-1}, 21 \citep{bonfilsetal07-1}, 22 \citep{bonfilsetal18-1}, 23 \citep{butleretal06-1}, 24 \citep{montetetal14-1}, 25 \citep{gillonetal16-1}. 26 \citep{grimetal18-1} }
\tablenotetext{a}{Optical activity designation where ``Y'' (Yes) indicates targets for which H$\alpha$ is in emission \citep{newtonetal17-1} }
\tablenotetext{b}{M$\sin i$ }
\end{deluxetable}

\begin{table}[]
    \centering
    \begin{tabular}{l c c c c } \hline \hline
     Name & $L_{\mathrm{bol}}$ (10$^{31}$ erg s$^{-1}$)  & Mass ($M_{\odot}$) & Radius ($R_{\odot}$) & $T_{\mathrm{eff}}$ (K) \\ \hline
	TRAPPIST-1 & $0.234 \pm ^{0.009}_{0.008}$ & $0.090 \pm ^{0.003}_{0.002}$ & $0.120 \pm 0.006 $ & $2619 \pm ^{71}_{66}$ \\ 
	LHS 2686 & $1.078 \pm 0.024$ & $0.157 \pm 0.004$ & $0.182 \pm 0.008 $ & $3119 \pm ^{70}_{68}$ \\ 
	GJ 699  & $1.302 \pm ^{0.024}_{0.023}$ & $0.1610 \pm ^{0.0036}_{0.0035} $ & $0.187 \pm 0.001$ & $3223 \pm 17 $ \\ 
	GJ 729 & $1.537 \pm 0.018$ & $0.177 \pm 0.004 $ & $0.200 \pm 0.008 $ & $3248 \pm ^{68}_{66}$ \\ 
	GJ 1132 & $1.668 \pm ^{0.049}_{0.047}$ & $0.194 \pm 0.005$ & $0.215 \pm 0.009$ & $3196 \pm ^{71}_{70}$ \\ 
	L 980-5 & $2.488 \pm ^{0.079}_{0.078}$ & $0.232 \pm 0.006$ & $0.250 \pm 0.010$ & $3278 \pm ^{74}_{70}$ \\ 
	GJ 674  & $6.03 \pm 0.14 $ & $0.353 \pm 0.008$ & $0.361 \pm ^{0.012}_{0.011}$ & $3404 \pm ^{59}_{57}$ \\ 
	GJ 15A  & $8.608 \pm 0.069$ & $0.393 \pm ^{0.009}_{0.008}$ & $0.385 \pm0.002$ & $3601 \pm ^{12}_{11}$ \\ 
	GJ 163 & $8.28 \pm 0.24$ & $0.405 \pm 0.010 $ & $0.409 \pm ^{0.017}_{0.016}$ & $3460 \pm ^{76}_{74}$ \\ 
	GJ 849 & $11.051 \pm ^{0.095}_{0.094}$ & $0.465 \pm 0.011$ & $0.464 \pm 0.018$ & $3492 \pm ^{70}_{68}$ \\ 
	GJ 649  & $16.74 \pm 0.170 $ & $0.524 \pm 0.012 $ & $0.531 \pm 0.012 $ & $3621 \pm ^{41}_{40}$ \\ 
	GJ 676A & $34.04 \pm ^{0.84}_{0.80}$ & $0.631 \pm 0.017$ & $0.617 \pm ^{0.028}_{0.027}$ & $4014 \pm ^{94}_{90}$ \\ \hline
    \end{tabular}
    \caption{Stellar parameters for the Mega-MUSCLES sample reproduced from Table 3 of \citet{pinedaetal21-1}.}
    \label{tab:params}
\end{table}

==> line_list.tex <==

% \begin{table*}
% % \begin{center}
    
% \vspace{1in}

% \begin{rotatetable*}

%     \centering
    
%     \begin{tabular}{lcccccccccc} \hline \hline
%      & \multicolumn{10}{c}{Line Flux (10$^{-16}$ erg s$^{-1}$ cm$^{-2}$)}\\
%     & Si III & O V & N Vm & Fe XII & S II & Si II & C IIm & Fe XXI & Si IVm & C IVm\\
%   Star& 1206.499\,\AA & 1218.39\,\AA & 1240.0\,\AA & 1242.0\,\AA & 1253.811\,\AA & 1309.27\,\AA & 1335.0\,\AA & 1354.08\,\AA & 1400.0\,\AA & 1550.0\,\AA\\
%   \hline
% GJ 1132 & 0.21$\pm$0.01 & \nodata & 0.25$\pm$0.12 & \nodata & \nodata & \nodata & 0.63$\pm$0.03 & \nodata & 0.07$\pm$0.01 & 1.23$\pm$0.87\\
% GJ 15A & 202.15$\pm$3.41 & 119.8$\pm$1.18 & & 294.4$\pm$2.1 & 9.18$\pm$0.45 & 32.0$\pm$1.96 & & 208.10$\pm$6.15 & 1119.30$\pm$8.18\\
% GJ 163 & 6.91$\pm$2.00 & 0.44$\pm$0.03 & 0.63$\pm$0.02 & 0.63$\pm$0.02 & \nodata & \nodata & 1.95$\pm$0.04 & $<$1.50 & \nodata & 0.70$\pm$0.04\\
% GJ 649 & \nodata & 1.01$\pm$10.08 & 24.93$\pm$0.17 & 24.93$\pm$0.17 & \nodata & \nodata & 44.36$\pm$0.17 & $<$1.73 & \nodata & 65.56$\pm$3.28\\
% GJ 674 & 77.80$\pm$0.37 & \nodata & 121.14$\pm$0.52 & 121.14$\pm$0.52 & \nodata & \nodata & 116.90$\pm$0.44 & $<$0.17 & \nodata & \\
% GJ 676A & \nodata & 5.25$\pm$0.53 & 48.05$\pm$0.23 & 48.05$\pm$0.23 & \nodata & 1.59$\pm$15.85 & 72.10$\pm$7.21 & $<$1.03 & 4.95$\pm$1.36 & 88.44$\pm$8.84\\
% Barnard\'s Star & 14.39$\pm$1.25 & \nodata & 31.49$\pm$0.61 & 31.49$\pm$0.61 & 0.02$\pm$0.16 & 0.35$\pm$0.06 & 50.65$\pm$1.25 & $<$0.24 & \nodata & \\
% GJ 729 & 28.98$\pm$1.50 & 7.50$\pm$0.69 & \nodata & \nodata & \nodata & \nodata & 34.66$\pm$0.67 & \nodata & \nodata & 65.59$\pm$2.08\\
% GJ 849 & $<$0.27 & 5.97$\pm$0.06 & 44.81$\pm$0.21 & 44.81$\pm$0.21 & \nodata & \nodata & 44.73$\pm$0.09 & \nodata & \nodata & 33.26$\pm$0.39\\
% GJ 876 & 27.62$\pm$2.67 & 17.38$\pm$1.60 & 47.12$\pm$4.03 & 47.12$\pm$4.03 & \nodata & \nodata & 56.41$\pm$5.59 & \nodata & 2.07$\pm$0.21 & 158.88$\pm$12.01\\
% L-980-5 & 0.77$\pm$0.05 & $<$1.03 & 0.87$\pm$0.06 & 0.87$\pm$0.06 & \nodata & \nodata & 0.98$\pm$0.02 & \nodata & \nodata & 6.30$\pm$4.52\\
% LHS-2686 & 7.17$\pm$0.09 & \nodata & 22.26$\pm$0.23 & 22.26$\pm$0.23 & \nodata & \nodata & 16.05$\pm$0.20 & \nodata & \nodata & \\
% TRAPPIST-1 & \nodata & \nodata & 0.52$\pm$0.12 & 0.52$\pm$0.12 & \nodata & 0.06$\pm$0.03 & \nodata & \nodata & \nodata & 1.53$\pm$0.49\\
% \hline

%     \end{tabular}



% \caption{List of FUV emission line flux measurements used to  create the DEMs. Lines marked ``m'' are multipets where the given wavelength is the approximate midpoint. }
% \label{tab:linelist}

% \end{rotatetable*}
% \end{center}

% \end{table}




\begin{rotatetable}
% \movetabledown=10mm
\movetableright=0.01mm

\begin{deluxetable*}{lcccccccccc}
\tablecaption{List of FUV emission line flux measurements used to  create the DEMs. Lines marked ``m'' are multiplets where the given wavelength is the approximate midpoint.\label{tab:linelist}}
% \tabletypesize{}
\tablecolumns{11}
 \tablehead{\colhead{} & \multicolumn{10}{c}{Line Flux (10$^{-16}$ erg s$^{-1}$ cm$^{-2}$)}\\
 \colhead{} & \colhead{Si III} & \colhead{O V} & \colhead{N Vm} & \colhead{Fe XII} & \colhead{S II} & \colhead{Si II} & \colhead{C IIm} & \colhead{Fe XXI} & \colhead{Si IVm} & \colhead{C IVm} \\
 \colhead{Star}& \colhead{1206.499\,\AA} & \colhead{1218.39\,\AA} & \colhead{1240.0\,\AA} & \colhead{1242.0\,\AA} & \colhead{1253.811\,\AA} & \colhead{1309.27\,\AA} & \colhead{1335.0\,\AA} & \colhead{1354.08\,\AA} & \colhead{1400.0\,\AA} & \colhead{1550.0\,\AA}}
\startdata
GJ\,1132 & 0.21$\pm$0.01 & \nodata & 0.25$\pm$0.12 & \nodata & \nodata & \nodata & 0.63$\pm$0.03 & \nodata & 0.07$\pm$0.01 & 1.23$\pm$0.87\\
GJ\,15A & 202.15$\pm$3.41 & 119.8$\pm$1.18 & & 294.4$\pm$2.1 & 9.18$\pm$0.45 & 32.0$\pm$1.96 & & 208.10$\pm$6.15 & 1119.30$\pm$8.18\\
GJ\,163 & 6.91$\pm$2.00 & 0.44$\pm$0.03 & 0.63$\pm$0.02 & 0.63$\pm$0.02 & \nodata & \nodata & 1.95$\pm$0.04 & $<$1.50 & \nodata & 0.70$\pm$0.04\\
GJ\,649 & \nodata & 1.01$\pm$10.08 & 24.93$\pm$0.17 & 24.93$\pm$0.17 & \nodata & \nodata & 44.36$\pm$0.17 & $<$1.73 & \nodata & 65.56$\pm$3.28\\
GJ\,674 & 77.80$\pm$0.37 & \nodata & 121.14$\pm$0.52 & 121.14$\pm$0.52 & \nodata & \nodata & 116.90$\pm$0.44 & $<$0.17 & \nodata & \\
GJ\,676A & \nodata & 5.25$\pm$0.53 & 48.05$\pm$0.23 & 48.05$\pm$0.23 & \nodata & 1.59$\pm$15.85 & 72.10$\pm$7.21 & $<$1.03 & 4.95$\pm$1.36 & 88.44$\pm$8.84\\
GJ\,699 & 14.39$\pm$1.25 & \nodata & 31.49$\pm$0.61 & 31.49$\pm$0.61 & 0.02$\pm$0.16 & 0.35$\pm$0.06 & 50.65$\pm$1.25 & $<$0.24 & \nodata & \\
GJ\,729 & 28.98$\pm$1.50 & 7.50$\pm$0.69 & \nodata & \nodata & \nodata & \nodata & 34.66$\pm$0.67 & \nodata & \nodata & 65.59$\pm$2.08\\
GJ\,849 & $<$0.27 & 5.97$\pm$0.06 & 44.81$\pm$0.21 & 44.81$\pm$0.21 & \nodata & \nodata & 44.73$\pm$0.09 & \nodata & \nodata & 33.26$\pm$0.39\\
GJ\,876 & 27.62$\pm$2.67 & 17.38$\pm$1.60 & 47.12$\pm$4.03 & 47.12$\pm$4.03 & \nodata & \nodata & 56.41$\pm$5.59 & \nodata & 2.07$\pm$0.21 & 158.88$\pm$12.01\\
L-980-5 & 0.77$\pm$0.05 & $<$1.03 & 0.87$\pm$0.06 & 0.87$\pm$0.06 & \nodata & \nodata & 0.98$\pm$0.02 & \nodata & \nodata & 6.30$\pm$4.52\\
LHS-2686 & 7.17$\pm$0.09 & \nodata & 22.26$\pm$0.23 & 22.26$\pm$0.23 & \nodata & \nodata & 16.05$\pm$0.20 & \nodata & \nodata & \\
TRAPPIST-1 & \nodata & \nodata & 0.52$\pm$0.12 & 0.52$\pm$0.12 & \nodata & 0.06$\pm$0.03 & \nodata & \nodata & \nodata & 1.53$\pm$0.49\\
\hline
\enddata
\end{deluxetable*}

\end{rotatetable}

